FedDUAP: Federated Learning with Dynamic Update and Adaptive Pruning Using Shared Data on the Server

Despite achieving remarkable performance, Federated Learning (FL) suffers from two critical challenges, i.e., limited computational resources and low training efficiency. In this paper, we propose a novel FL framework, i.e., FedDUAP, with two original contributions, to exploit the insensitive data on the server and the decentralized data in edge devices to further improve the training efficiency. First, a dynamic server update algorithm is designed to exploit the insensitive data on the server, in order to dynamically determine the optimal steps of the server update for improving the convergence and accuracy of the global model. Second, a layer-adaptive model pruning method is developed to perform unique pruning operations adapted to the different dimensions and importance of multiple layers, to achieve a good balance between efficiency and effectiveness. By integrating the two original techniques together, our proposed FL model, FedDUAP, significantly outperforms baseline approaches in terms of accuracy (up to 4.8% higher), efficiency (up to 2.8 times faster), and computational cost (up to 61.9% smaller).

==> backup.tex <==
%Even if not to mention these devices with strong computation capabilities, with the realization of smart home and intelligent transportation, Internet of things devices are also very common in our life. Most of these devices have certain computation and storage capabilities. While they bring a lot of convenience to our life, they also generate and store a large amount of data. In order to make these devices have a certain intelligence, machine learning technology is very important. From speech recognition to face recognition, artificial intelligence models all need a large amount of data, and these edge devices can provide such huge data. Therefore, people have long proposed mobile edge computing (MEC) frameworks to use these data to train models~\cite{hu2015mobile}.

%MEC frameworks require edge devices to upload local data to the server, and finally train a model with all data by the server. This brings two problems. On the one hand, the number of edge devices is very large, and the amount of data generated is also difficult to estimate. Uploading these data will undoubtedly bring considerable pressure to the network. On the other hand, not to mention that most of the data is private, and the data owners are unwilling to upload these data. Even if the data center commits to protect these data, it will face malicious attacks in the process of transmission. Moreover, for the central server, the cost of storing so much data is high.

%To address the private and communication problems mentioned above, McMahan~\shortcite{mcmahan2017communication} proposed Federated Learning (FL) framework. FL framework is different from MEC frameworks, and it is an iterative process. In each iteration, 1) the server randomly selects a certain number of devices and sends the global model to all the selected devices. 2) The selected devices update the global model with local data and upload the updated model after training. 3) The server aggregates all uploaded local models to form a new global model. FL repeats this iterative process until the model finally converges. In the whole process of model training, the data remains in the edge device, so the privacy of the data is guaranteed. At the same time, in the process of FL, there is no need to upload data, but only upload and download relatively small model parameters, which greatly reduces the pressure of communication.

%We do not need to introduce the security or privacy in federated learning, as this is not our main contribution.
%The MEC framework is proposed to provide a solution for how to use data on edge devices training artificial intelligence models, but it also brings privacy and communication problems. In order to solve these two problems, FL protocol is proposed to let devices train the model locally, which ensures the security of local data and does not consume a lot of communication resources to transmit local data, but FL also has its own problems. The research on FL mainly focuses on two aspects: privacy security and training efficiency. Privacy security can be divided into two aspects: privacy and security. For privacy, although the strategy of not uploading local data in FL protects the privacy of data to a certain extent, it still needs to upload the locally updated model in the process of FL, which gives other participants the opportunities to infer sensitive information. Common technologies to solve privacy problems include differential privacy~\cite{ma2020safeguarding,liu2018epic,du2018big}and secure aggregation~\cite{bonawitz2017practical,bonawitz2016practical,truex2019hybrid}. Another aspect is security. In the process of FL, there will be some attacks, which will lead to the deterioration in the model's performance or failure in the training process. The attacks are mainly divided into two categories: target attacks and untargeted attacks. For security attacks, there are three main techniques, which are security analysis~\cite{bhagoji2019analyzing,bagdasaryan2020backdoor}, statics~\cite{munoz2019byzantine,fung2018mitigating} and autoencoders~\cite{yu2017recursive}.


% Not related
%Another research focus of FL is training efficiency, which is also the research aspect of our paper, and there are many factors affecting training efficiency. Because different devices have different resources, this resource gap will lead to the difference in the time for completing a round of training, and even some devices can not complete the task within the specified time. Therefore, it is necessary to coordinate the scheduling among devices in FL according to the resources of different devices, and that's what~\cite{nishio2019client} does. By considering the computation, communication, and battery resources of the devices,~\cite{nishio2019client} better selects the devices for each round of training, reduces the training time of each round, and finally speeds up the convergence efficiency of FL.~\cite{wu2020safa} further considers the instability of devices on the basis of~\cite{nishio2019client}.

% not related
%The above methods are synchronous. Synchronous means that in a round of training, the aggregation of FL only uses the local model updated by the current round of devices. Obviously, this is not efficient enough, and the resources of many other devices are not used reasonably. Therefore,~\cite{xie2019asynchronous} proposes an asynchronous federated update method from the perspective of communication. In~\cite{xie2019asynchronous}, the current round of federated aggregation will not only use the devices selected in the current round, but also the devices that have not completed the task in the previous rounds, thus improving the utilization of devices resources.

%~\cite{briggs2020federated} groups the devices according to the similarity of model gradients, and each group trains a model separately. However, this approach contradicts the original vision of FL, which expects each device to be treated equally and to train one single model uniformly.~\cite{duan2019astraea} adopts data augmentation and scheduling aggregation to solve the global imbalance problem. Starting from the training of the model,~\cite{li2018federated} adds an approximate term to the objective function of the model, which restricts the training of the model from deviating too much from the original model, which well suppresses the excessive deviation of the model trained under non-IID data.~\cite{zhao2018federated} starts from the data and assumes that there is a globally shared IID dataset on the server. Then~\cite{zhao2018federated} distributes the dataset to all devices, allowing them to train on the mixed datasets. However,~\cite{yoshida2020hybrid} thinks it is difficult to have such a large public dataset, thus proposing to pay to obtain data from some devices to form a globally shared IID dataset. Unlike~\cite{zhao2018federated},~\cite{yoshida2020hybrid} chooses to train a model on the server with the globally shared IID dataset and let the model participate in the aggregation process. Even if some devices are willing to upload a segment of data, uploading data will undoubtedly bring a lot of overhead to communication. Different from~\cite{zhao2018federated} and~\cite{yoshida2020hybrid},~\cite{jeong2018communication} requires devices to upload some sample data of missing labels, then train a GAN on the server, and send the generated GAN generator to devices, so that the devices can build samples of missing labels, forming the local IID data. Only uploading some samples and GAN generator undoubtedly reduce the communication, but even so, there will be certain communication pressure.

%The key idea of our algorithm is to optimize the aggregated model on the server by using the globally shared dataset. For server model adjustment, if edge devices have a non-IID dataset, FedGMS will adjust the aggregated model through the relatively well distributed shared data, which can effectively limit the negative impacts of data heterogeneity, thus accelerating its convergence speed. Even if edge devices have an IID dataset, FedGMS will make additional updates to the aggregated model on the globally shared dataset, which will also undoubtedly accelerate the convergence speed of the model in one round. In our hypothesis, the server has relatively strong computation capabilities compared to edge devices, so the time of server model adjustment can be negligible in a round. Since FedGMS accelerates the convergence effect of each round, and the time of each round is not different from that of other FL algorithms, the overall convergence speed can be improved. In addition, we use shared data to prune the model during training, which reduces the number of model parameters and computation with little impact on model performance, thus speeding up the efficiency of FL.

% \begin{algorithm}[h]
% \floatname{algorithm}{Protocol}
% \caption{FedGMS Protocol.}
% \begin{algorithmic}[1]
% \STATE \emph{Initialization}: The server initializes a global model randomly.\
% \STATE \emph{Client Selection}: The server randomly selects $m$ devices from $N$ devices to participate in the current round task.
% \STATE \emph{Distribution}: The server distributes the parameters of the global model to the selected devices.
% \STATE \emph{Update and Upload}: Each selected device updates the global model with local data and uploads the updated model parameters to the server.
% \STATE \emph{Aggregation}: If the server gets all the updated parameters, it averages them and get the aggregated model.
% \STATE \emph{Server Adjustment}: The server uses globally shared data to adjust the aggregated model to obtain a new global model.
% \STATE All steps but \emph{Initialization} are iterated until the global model achieves the desired performance or the final deadline arrives.
% \end{algorithmic}
% \label{code:fedgms}
% \end{algorithm}

%We show FedGMS in algorithm \ref{code:fedgms} and Figure \ref{fig:framework}. Compared with FedAvg, most of the steps of FedGMS are the same. The difference is that there are additional steps for server model adjustment and model pruning. 

%We adjust the aggregated model on the server by using the globally shared data. On the one hand, we speed up the convergence speed of the model by relying on the advantages of the server's computation capabilities to carry out more training. On the other hand, we balance the impact of the non-IID data of the edge device by the relatively well distributed shared data. However, the adjustment of the server also brings some problems. If the server adjusts the global model too much, the model will be completely offset to the server data, and it becomes difficult for the model to obtain the performance improvement brought by the edge device data, and even damage the overall model performance. If the server adjusts too little, then globally shared data is not utilized enough to bring a speed increase to the overall FL process. To this end, we used two strategies.

%Due to the different amount of shared data, the number of update iterations (or steps) varies with the same batch size $B$ and epoch $E$. Excessive iterations will cause the model to shift to shared data. To avoid manually specifying the number of central iterations for different scenarios, we normalize the gradient~\cite{wang2020tackling}. Because the distribution of central data is better than that of edge devices, more iterations can determine a good direction for the model and serve as a guide for global update. And we specify a small step size in this direction to make a fine tuning of the global model. The server normalized gradient can be calculated as follows:

%where $w^{t-,i}$ is the weight parameter of the $i$-th update iteration of the aggregated model in round $t$, $g(\cdot)$ represents the corresponding gradient, and $\tau =\lceil \frac{|\mathcal{D}_0| E}{B} \rceil$ is the number of update iterations performed by the server. Then we updated the aggregated model with effective steps $\tau_{eff}^t$ as follows:
%\begin{equation}
%w^t = w^{t-} - \tau_{eff}^t\eta \overline{g}^{(t)}
%\end{equation}

%Although a small fixed number of effective steps $\tau_{eff}$ can help fine-tune the model to achieve a better result, we still want to use the available information  to dynamically adjust $\tau_{eff}$. A simple idea is that at the initial stage of FL, we make more adjustments on the server to help the model achieve certain performance quickly and accelerate the convergence speed of the model. In the middle and later stages of FL, since the model has reached a certain performance, we want the model to make more use of the data of edge devices for further optimization and improvement, and reduce the intervention of server adjustment. Therefore, we introduce a dynamic adjustment strategy for determining $\tau_{eff}$ each round as shown in Algorithm \ref{alg:dyamic}.

%Firstly, we evaluate the current aggregated model on the central data to obtain an accuracy $acc$, which can reflect the performance of the current model to a certain extent, and $\tau_{eff}$ will be inversely correlated to it. It is worth mentioning that when accuracy is low, such as $acc=0.2$, and when accuracy increases to a certain level, such as $acc=0.8$, $\tau_{eff}$ will be 4 times different. This is also consistent with our idea to help the model achieve certain performance quickly at the beginning of FL.

%At the same time, we also consider the data distribution. When participating devices' data distribution of current round is good or the central data distribution is poor, we will reduce the server intervention. We use a relative value between the two to adjust the coefficient, while considering the corresponding data quantity relationship.

%Additionally, we add a hyperparameter $decay$  to reduce server interference in the later stage of FL. $decay$  has a value between 0 and 1, and when this value is small, the server reduces intervention earlier. When $decay=0$, the dynamic iteration algorithm degenerates into FedAvg.

%Finally, we multiply the various coefficients by the average number of iterations of the current round devices to get $\tau_{eff}$.

% \subsubsection{Server Training Constraints}
% In order to prevent the adjustment of the server from greatly deviating from the aggregated model, we have made some minor adjustments to the optimization function of the server. We introduce a penalty term~\cite{li2018federated}, and the optimization function of the server in round $t$ is as follows:
% \begin{equation}
% \min_{w}F_0(w)\triangleq\frac{1}{n_0}\sum_{\{x_{0,j},y_{0,j}\} \in \mathcal{D}_0} f(w,x_{0,j},y_{0,j}) + \frac{\mu}{2}\left\|w - w^{t-}\right\|^2
% \end{equation}
% where $\mu$ is the regularization weight parameter, $n_0$ represents the number of globally shared data, $\mathcal{D}_0$ represents the globally shared dataset, and $w^{t-}$ represents the model after $t$-th round aggregation. The penalty term limits the server's adjustment to be close to the aggregated model, which will reduce the server's overtraining and make the convergence of the model more stable.

%It can be seen that compared with Data-sharing, from the perspective of round, due to the huge increase in the amount of edge data in Data-sharing, the accuracy of this method increases very quickly. However, considering that this method needs to transmit a large amount of data, on the one hand, it requires a certain amount of communication, and on the other hand, it also increases the calculation amount of edge devices, which leads to much more time in each round than \TheName{}-D. From the perspective of time, the overall convergence speed of Data-sharing is not as fast as \TheName{}-D. From the perspective of the accuracy of final convergence, because Data-sharing makes full use of all shared data, the accuracy is ultimately 1.1\% higher in the case of CNN. However, in the case of VGG, \TheName{}-D is better than Data-sharing by 2\%. It is speculated that the fitting ability of VGG model is better, and finally there is too much fitting for shared data. In addition, it is not practical to transfer all shared data to all devices, and \TheName{}-D will also have an advantage in the case of small data transfer volumes. Compared with Hybrid-FL, the convergence speed of \TheName{}-D is similar , but the final convergence accuracy has certain advantages about 2\% in some cases.

% \begin{table*}[htbp]
% \caption{\textbf{Results obtained for FedAvg and FedGMS with IID and non-IID settings.} ToA@x: the round required to arrive at a testing classification accuracy of x. Accuracy: the best test accuracy in the training. NaN means that the method did not achieve the required accuracy.}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Method}}} &\multicolumn{4}{|c|}{\textbf{Time}} \\
% \cline{3-6} 
% \multicolumn{2}{|c|}{} &\textbf{\textit{ToA@0.5}}& \textbf{\textit{ToA@0.55}}& \textbf{\textit{ToA@0.6}} &\textbf{\textit{Accuracy}}  \\
% \hline
% \multirow{4}{*}{\textbf{IID}}& \textbf{FedAvg} & 36& 58& 130& 0.62\\
% \cline{2-6} 
% & \textbf{FedGMS (p=1\%)} & 33& 53& 106& 0.62\\
% \cline{2-6} 
% & \textbf{FedGMS (p=5\%)} & 26& 44& 90& 0.62\\
% \cline{2-6} 
% & \textbf{FedGMS (p=10\%)} & 21& 33& 63& 0.64\\
% \hline
% \multirow{4}{*}{\textbf{non-IID}}& \textbf{FedAvg} & 238 & NaN & NaN & 0.53\\
% \cline{2-6} 
% & \textbf{FedGMS (p=1\%)} & 160 & NaN & NaN & 0.54\\
% \cline{2-6} 
% & \textbf{FedGMS (p=5\%)} & 73 & 145 & NaN & 0.59\\
% \cline{2-6} 
% & \textbf{FedGMS (p=10\%)} & 48 & 88 & 227 & 0.61\\
% \hline
% \end{tabular}
% \label{tab1}
% \end{center}
% \end{table*}


\begin{algorithm}[h]
\caption{FedGMS (Proposed Framework) }
\label{code:fedgms}
\leftline{\textbf{Server process:} \quad //running on the server}
\begin{algorithmic}[1]
\REQUIRE  \quad \\
$T$: The number of global rounds \\
$\mu$: The learning rate \\
$w^0$: The initial model parameters
\FOR{$t=1,\cdots, T$}
\STATE $\mathcal{S}_t \leftarrow$ Randomly select device set for current round training
\FOR{each device $k \in \mathcal{S}_t$ in parallel}
\STATE $w_k^{t} \leftarrow DeviceUpdate(k, w^{t-1})$
\ENDFOR
\STATE  Server aggregates the $w$'s as $w^{t-} \leftarrow \frac{1}{\sum_{k \in \mathcal{S}_t} |\mathcal{D}_k|}\sum_{k \in \mathcal{S}_t}|\mathcal{D}_k|w_k^t$
\STATE Call \textbf{Algorithm 2} with $\mathcal{S}_t$, $w^{t-}$ and $decay$ to get $\tau_{eff}$
\STATE $w^t \leftarrow ServerUpdate(w^{t-}, \tau_{eff})$
\STATE Perform pruning according to \textbf{Algorithm 3} 
\ENDFOR
\end{algorithmic}

\leftline{\textbf{Device Update:} \quad //running on the selected device $k$}
\begin{algorithmic}[1]
\REQUIRE  \quad \\
$w^{t-1}$: The global model parameters in round $t-1$
\ENSURE \quad \\
$w_k^{t}$: The updated model parameters on device $k$
\STATE $w \leftarrow w^{t-1}$
\STATE $\mathcal{X}_k \leftarrow$ Split $\mathcal{D}_k$ into batches of size $B$
\FOR{each local epoch $i$ from $1$ to $E$}
\FOR{batch $x_k \in \mathcal{X}_k$ }
\STATE $w \leftarrow w - \eta\nabla F(w,x_k)$
\ENDFOR
\ENDFOR
\end{algorithmic}
\leftline{\textbf{Server Update:} \quad //running on the server}
\begin{algorithmic}[1]
\REQUIRE  \quad \\
$w^{t-}$: The aggregated model parameters in round $t$ \\
$\tau_{eff}$: The effective steps
\ENSURE \quad \\
$w^{t}$: The updated model parameters on the server
\STATE $w \leftarrow w^{t-}$
\STATE $\mathcal{X}_0 \leftarrow$ Split $\mathcal{D}_0$ into batches of size $B$
\FOR{each local epoch $i$ from $1$ to $E$}
\FOR{batch $x_k \in \mathcal{X}_0$ }
\STATE $w \leftarrow w - \eta\nabla F(w,x_k)$
\ENDFOR
\ENDFOR
\STATE $\overline{g}^{(t)} \leftarrow \frac{(w - w^{t-})*B}{|\mathcal{D}_0|*E}$
\STATE $w \leftarrow w^{t-} + \overline{g}^{(t)} * \tau_{eff}$
\end{algorithmic}
\end{algorithm}
